Enabling Resource-efficient AIoT System with Cross-level Optimization: A survey

The emerging field of artificial intelligence of things (AIoT, AI+IoT) is driven by the widespread use of intelligent infrastructures and the impressive success of deep learning (DL). With the deployment of DL on various intelligent infrastructures featuring rich sensors and weak DL computing capabilities, a diverse range of AIoT applications has become possible. However, DL models are notoriously resource-intensive. Existing research strives to realize near-/realtime inference of AIoT live data and low-cost training using AIoT datasets on resource-scare infrastructures. Accordingly, the accuracy and responsiveness of DL models are bounded by resource availability. To this end, the algorithm-system co-design that jointly optimizes the resource-friendly DL models and model-adaptive system scheduling improves the runtime resource availability and thus pushes the performance boundary set by the standalone level. Unlike previous surveys on resource-friendly DL models or hand-crafted DL compilers/frameworks with partially fine-tuned components, this survey aims to provide a broader optimization space for more free resource-performance tradeoffs. The cross-level optimization landscape involves various granularity, including the DL model, computation graph, operator, memory schedule, and hardware instructor in both on-device and distributed paradigms. Furthermore, due to the dynamic nature of AIoT context, which includes heterogeneous hardware, agnostic sensing data, varying user-specified performance demands, and resource constraints, this survey explores the context-aware inter-/intra-device controllers for automatic cross-level adaptation. Additionally, we identify some potential directions for resource-efficient AIoT systems. By consolidating problems and techniques scattered over diverse levels, we aim to help readers understand their connections and stimulate further discussions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes


==> body/compiler.tex <==




==> body/primer.tex <==
\section{Primer of DNN Deployment}

%%%%%%%%%  先介绍一段深度模型如何部署，训练、推理在AIoT设备上如何实现的基本流程。存在哪些难度。

\subsection{DNN Computational Graph}
The DNN computational graph is the .
The topology of early neural networks was simple, and the machine learning framework can use simple configuration files to express their model structure (\eg the Buffer format in Caffe). 
With the rapid development of deep neural networks (DNNs), the computational graph emerges as a novel data structure representing the DNN computational logic and state in the training and inference phases. 
Specifically, the computational graph mainly provides the following key functions for the deep learning (DL) framework:
\begin{itemize}
    \item \textit{Unified expression for the input data, operators, and operator execution order of diverse DNN models}. 
    With this unified intermediate representation, users can write DNN programs in \textit{different high-level programming languages} (\eg Python, Julia, and C++) and support the execution of the underlying C and C++ operators over \textit{various target devices}.
    \item \textit{Accurate expression for the life cycle of intermediate variables}. 
    DL framework generates a large number of intermediate variables (\eg activation values and gradients passed between layers). 
    However, the lifetime of most intermediate variables is short-lived, except for DNN parameters which need to be persisted to the subsequent inference phase. 
    Therefore, based on the computational graph, the DL framework can accurately analyze the life cycle of the intermediate state (\ie, when they are created and destroyed), thereby helping the DL framework to manage memory.
    \item \textit{Presentation of operator execution dependencies in forward-propagating $\&$ back-propagating.}
    The computational graph can present the execution dependencies of DNN operators, thereby helping the DL framework find opportunities to execute operators asynchronously and improve the training/inference efficiency.
\end{itemize}

The DL platforms always employ a directed acyclic graph (DAG) for representing their computational graph.
%
The nodes in the graph represent the operators that are applied directly on the data flowing in and out through the edges.
%
The DNN computational graph includes the following key components. 

\begin{itemize}
    \item \textit{Tensor}. Tensor is the basic data structure.
    \begin{itemize}
        \item \textit{Input data}.
        \item \textit{Intermediate variables and their lifetime}.
    \end{itemize}
    \item \textit{Operator}. Operator is the basic operation unit.
    The DNN operators include four types.
    \begin{itemize}
        \item Tensor operators.
        \item Neural network operators.
        \item Data flow operators. 
        \item Control flow operators.
    \end{itemize} 
\end{itemize}


\begin{figure*}[t]
  \centering
    \subfloat[Static computational graph]{\label{fig:static_graph}
    \includegraphics[height=0.12\textwidth]{static_graph.pdf}}
    \hspace{5pt}
    \subfloat[Dynamic computational graph]{\label{fig:static_graph}
    \includegraphics[height=0.12\textwidth]{dynamic_graph.pdf}}
    %\vspace{-3mm}
\caption{Illustration of the difference between static and dynamic computational graph.}
\label{fig:graph}
%\vspace{-3mm}
\end{figure*}

\textbf{Static computation graph (\eg in TensorFlow) $\&$ dynamic computation graph (\eg in Pytorch)}.
%
% There is a difference between how they let their data and calculations flow through the graph, although both them 
%
The difference between static and dynamic graph scheme are illustrated in Figure \ref{fig:graph}.

\begin{itemize}
    \item \textit{Static Graph Optimization}. 
    The static graph scheme is compiled first and then executed.
    It is completely processed by the DL framework (\eg TensorFlow) without using the frontend language (\eg Python) interpreter.
    \begin{itemize}
        % \item \textbf{Properties of nodes $\&$ edges}.
        \item \textbf{Advantages}. 
        Since the graph is static, it provides many possibilities of optimizations in structure and resource distribution.
        The computations are slightly faster than a dynamic graph because of the fixed structure.
        \item \textbf{Disadvantages}. 
        Scales poorly to variable dimension inputs For example, A CNN architecture with a static computation graph trained on $28\times{28}$ images cannot perform well on images of different sizes like $100\times{100}$ without a lot of pre-processing boilerplate code.
        \item \textbf{Optimization space}. We can transform the static graph into equivalent or more efficient graph structures through \textit{graph optimization strategies}. 
    \end{itemize}
    When performing \textit{DNN training or inference}, the graph receives input data and executes the operators in the optimized graph through the hardware scheduling to complete the task.
    %%%%%%%
    \item \textit{Dynamic Graph Optimization}.
    The dynamic graph scheme is executed while interpreting. 
    The interpreter of the frontend language (\eg python) is used to parse the code. 
    And then the operator arrangement function of the  framework (\eg Pytorch) executes the operators within the dynamic graph to complete the task.
    \begin{itemize}
        % \item \textbf{Properties of nodes $\&$ edges}.
        \item \textbf{Advantages}. 
        Scalability to different dimensional input. 
        Scales very well for different dimensional inputs as a new pre-processing layer can be dynamically added to the DNN model.
        \item \textbf{Disadvantages}. 
        Allows very little space for graph optimization because a new graph needs to be created for each training instance/batch.
        \item \textbf{Optimization space}. 
        After we use the dynamic graph scheme to train the DNN parameters, we can convert the overall DNN architecture to the static graph format, and then serialize and save the DNN architecture and parameter files~\cite{}. 
        In this way, we can completely decouple the DNN inference process from the frontend code (\eg python), and expand the hardware support range of DNN deployment.
    \end{itemize}
\end{itemize}
% 动态图优化模式
%
% 静态图优化模式

\textbf{Back-propagation computation graph (\eg in TensorFlow) $\&$ forward-propagation computation graph (\eg in Pytorch)}.
\begin{itemize}
    \item \textit{Back-propagation Computation Graph Optimization}.
    \item \textit{Forward-propagation Computation Graph Optimization}.
\end{itemize}






\subsection{Diverse DNN Architectures}
%%%%%%%%% 介绍几种典型深度模型，每个三四行即可，指出其计算量、存储量对DNN部署的不同要求，列表格



\subsection{Non-uniform DNN Frameworks}
%%%%%%%%% 介绍几种典型深度模型框架，每个三四行即可，指出其对DNN部署的不同支撑，列表格




\subsection{Potential DNN Libraries on Various AIoT Devices}
%%%%%%%%% 介绍几种典型的AIoT设备及其对于深度模型部署在算力、存储单元方面的不同约束，每个三四行即可



\subsection{Framework Compiler Phases and MLIR}
The compiler converts the human-readable source code into computer-readable machine code with several layers of \textit{intermediate representation (IR)}.
And we xx
\begin{itemize}
    \item \textit{Intermediate representation (IR)} is the data structure used internally by a compiler to represent the source code~\cite{}. 
    And the IR should accurately represent the source code without loss of information and be independent of any particular source or target platform language.
    \item \textit{LLVM} is designed around the language-independent IR that can be optimized with a variety of transformations over multiple passes, as show in Figure \ref{fig:llvm}(a).
    \item \textit{Multi-Level Intermediate Representation (MLIR)} explores to build the \textit{reusable} and \textit{extensible} compiler infrastructures, to support DNN deployment on heterogeneous hardware, reduce the cost of building domain-specific compilers, and help bridge existing compilers, as illustrated in Figure \ref{fig:llvm}(b). 
    It unifies the infrastructures required to execute DNNs in various frameworks (\eg TensorFlow, pytorch) by defining a common intermediate representation (IR).
    Moreover, we can adopt multiple rounds of optimization in each intermediate representation layer. 
\end{itemize}



\begin{figure*}[t]
  \centering
    \subfloat[LLVM]{\label{fig:static_graph}
    \includegraphics[height=0.18\textwidth]{LLVM.pdf}}
    \hspace{7pt}
    \subfloat[MLIR]{\label{fig:static_graph}
    \includegraphics[height=0.18\textwidth]{MLIR.pdf}}
    %\vspace{-3mm}
\caption{Illustration of LLVM and MLIR in the compiler.}
\label{fig:llvm}
%\vspace{-3mm}
\end{figure*}


Figure \ref{fig:llvm}(b) illustrates an example of MLIR in TensorFlow. 
\TODO{figure}
The DNN computation graphs from TensorFlow can be run in the following diverse transmissions with MLIR.
\begin{itemize}
    \item Sending the graph to the TensorFlow executor. 
    \item Converting the graph to XLA HLO intermediate representation, which in turn invokes the LLVM for deploying on CPUs or GPUs, or continues to use XLA for TPU platform.
    \item Converting the graph to TensorRT, nGraph, or other compiler formats suitable for specific hardware instruction sets.
    \item Converting the graph to TensorFlow Lite format for executing at runtime.
    \item Converting the graph further via the Android Neural Network API (NNAPI) or related technologies to run on Android platforms.
\end{itemize}


We list some mainstream MLIR projects for DNN optimization and deployment provided by different frameworks as follows.
\begin{itemize}
    \item MLIR (in TensorFlow) ~\cite{}.
    \item Torch-MLIR (in Pytorch) ~\cite{}.
\end{itemize}

Thereby, previous efforts on xxxx  present xxxx.
\begin{itemize}
    \item \textit{DNN Compiler Frontend Optimization.}
    % \item \textit{LLVM Optimizer.}
    \item \textit{DNN Compiler Backend Optimization.}
\end{itemize}


\begin{figure*}[t]
  \centering
  \includegraphics[width=.92\textwidth]{framework.pdf}
  \caption{Illustration of the memory-aware DNN compiler and runtime optimization.}
  \label{fig:framework}
  \vspace{-3mm}
\end{figure*}


\subsection{The compiler phases in DL framework}
\begin{itemize}
    \item Compiler Front-end Optimization (Platform-independent). 
    The compiler front-end mainly analyzes and translates the user-given code to obtain the \textit{computational graph IR} and performs device-independent optimization on it.
    \item Compiler Back-end Optimization (Platform-dependent).
    The main responsibility of the compiler back-end  is to optimize further the IR issued by the front-end and finally generate a computation execution sequence that can be executed on the hardware.
    \begin{itemize}
        \item Node splitting and fusion.
        \item Operator selection and ranking.
        \item Memory allocation and scheduling.
    \end{itemize}
\end{itemize}

